Exploring Privacy and Security as Drivers for Environmental Sustainability in Cloud-Based Office Solutions (Extended Abstract)

This paper explores the intersection of privacy, cybersecurity, and environmental impacts, specifically energy consumption and carbon emissions, in cloud-based office solutions. We hypothesise that solutions that emphasise privacy and security are typically "greener" than solutions that are financed through data collection and advertising. To test our hypothesis, we first investigate how the underlying architectures and business models of these services, e.g., monetisation through (personalised) advertising, contribute to the services' environmental impact. We then explore commonly used methodologies and identify tools that facilitate environmental assessments of software systems. By combining these tools, we develop an approach to systematically assess the environmental footprint of the user-side of online services, which we apply to investigate and compare the influence of service design and ad-blocking technology on the emissions of common web-mail services. Our measurements of a limited selection of such services does not yet conclusively support or falsify our hypothesis regarding primary impacts. However, we are already able to identify the greener web-mail services on the user-side and continue the investigation towards conclusive assessment strategies for online office solutions.

==> Makefile <==

TEXFILES = index.tex abstract.tex acks.tex acros.tex


all: index.pdf

index.pdf: .FORCE sustainable-ict.bib tools.bib ${TEXFILES}
	latexmk -pdf index.tex

spelling: ${TEXFILES}
	for file in ${TEXFILES}; do \
          ispell -t -b -d british -p ./index.dict $$file; \
        done

index.tar.gz: index.pdf
	mkdir -p paper
	cp -r graphics paper/
	cp sustainable-ict.bib tools.bib index.bbl ${TEXFILES} paper/
	cp ACM-Reference-Format.bst acmart.cls paper/
	cp Makefile index.dict paper/
	cd paper && tar -cvf ../index.tar *
	gzip -9 index.tar
	rm -rf paper

.FORCE: spelling
	${MAKE} -C graphics/

clean:
	latexmk -c -pdf index.tex
	rm -rf paper index.tar index.tar.gz

distclean: clean
	rm -f index.pdf



==> graphics/Makefile <==
SVG_FILES   = $(shell ls -- *.svg)
GRAPHICS    = $(SVG_FILES:.svg=.pdf)

all: ${GRAPHICS}

%.pdf: %.svg Makefile
	inkscape --export-pdf=$@ $< \
          --export-text-to-path 
#          --export-background="#000000"

clean:
	rm -f ${GRAPHICS}

distclean: clean


